Retrieval-Augmented Egocentric Video Captioning

Understanding human actions from videos of first-person view poses significant challenges. Most prior approaches explore representation learning on egocentric videos only, while overlooking the potential benefit of exploiting existing large-scale third-person videos. In this paper, (1) we develop EgoInstructor, a retrieval-augmented multimodal captioning model that automatically retrieves semantically relevant third-person instructional videos to enhance the video captioning of egocentric videos. (2) For training the cross-view retrieval module, we devise an automatic pipeline to discover ego-exo video pairs from distinct large-scale egocentric and exocentric datasets. (3) We train the cross-view retrieval module with a novel EgoExoNCE loss that pulls egocentric and exocentric video features closer by aligning them to shared text features that describe similar actions. (4) Through extensive experiments, our cross-view retrieval module demonstrates superior performance across seven benchmarks. Regarding egocentric video captioning, EgoInstructor exhibits significant improvements by leveraging third-person videos as references. Project page is available at: https://jazzcharles.github.io/Egoinstructor/

==> caption_strategy.tex <==

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
  \begin{tabular}[t]{lccccc}
    \toprule
    Model & Strategy & BELU-4 & METEOR & ROUGE-L & CIDER \\
    \midrule
    MPT-1B & random & 0.010 & 0.071 & 0.182 & 0.054 \\
    MPT-1B & V2V & 0.022 & 0.122 & 0.231 & 0.216 \\
    MPT-1B & V2T & 0.023 & 0.128 & 0.235 & 0.239\\
    MPT-1B & V2V+V2T & 0.024 & 0.130 & 0.241 & 0.245 \\
    MPT-1B & GT & \textbf{0.032} &\textbf{ 0.153} & \textbf{0.261} & \textbf{0.327}\\
    \bottomrule
  \end{tabular}
}
\vspace{-5pt}
\caption{Comparison results of different retrieval strategies for captioning on EgoLearner. We report the 1-shot captioning performance.}
\label{tab:caption_strategy}
\end{table}

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
  \begin{tabular}[t]{lcccccc}
    \toprule
    \multirow{2}{*}{Retriever} & \multicolumn{2}{c}{EgoLearner-MCQ} & \multicolumn{4}{c}{EgoLearner-Captioning} \\
    \cmidrule(r){2-3}\cmidrule(r){4-7}
    & Ego2Exo & Exo2Ego & BELU-4 & METEOR & ROUGE-L & CIDER \\
    \midrule
    VideoMAE & 44.0 & 30.4 & 0.020 & 0.123 & 0.225 & 0.213 \\
    InternVideo & 52.8 & 48.3 & 0.024 & 0.130 & 0.241 & 0.245 \\
    \bottomrule
  \end{tabular}
}
\vspace{-5pt}
\caption{Comparison on different retrieval models for exocentric video selection.}
\label{tab:caption_model}
\end{table}

